A Survey on Artificial Intelligence for Source Code: A Dialogue Systems Perspective

In this survey paper, we overview major deep learning methods used in Natural Language Processing (NLP) and source code over the last 35 years. Next, we present a survey of the applications of Artificial Intelligence (AI) for source code, also known as Code Intelligence (CI) and Programming Language Processing (PLP). We survey over 287 publications and present a software-engineering centered taxonomy for CI placing each of the works into one category describing how it best assists the software development cycle. Then, we overview the field of conversational assistants and their applications in software engineering and education. Lastly, we highlight research opportunities at the intersection of AI for code and conversational assistants and provide future directions for researching conversational assistants with CI capabilities.

==> paper_sections/commented.tex <==


%  Section 3:
% DRAFT

% Seq2Seq:

% Our goal is to build a neural network that directly models the conditional probability $p(a|e)$ of translating an input sequence of natural language tokens, $e_1,...,e_e$, with length $|e|$ to a target sequence of assembly language tokens, $a_1,...,a_a$ with length $|a|$. As a simple example, consider the sequence of English tokens {\fontfamily{qcr} \small\selectfont
% [`add', `4', `to', `eax']} as $e$ and $a$ as {\fontfamily{qcr} \small \selectfont
% [`add', `eax', `,' , `4']} with $|e| = 4$ and $|a| = 4$.

% The basic sequence-to-sequence NMT system consists of an encoder, which computes a representation $s$ for each source token, and a decoder, which generates one target token at a time and hence decomposes the conditional probability as:
% % Maybe include a snippet tokenized as an example? See http://www.phontron.com/paper/oda15ase.pdf page 3

% \begin{equation}
% \label{eq:decoding}
% \log p(a|e) =\sum_{j=1}^{m} \log p(a_j|a_{<j},s)
% \end{equation}

% Given an English intent $e$, our decoding problem is to find an assembly token sequence $\hat{a}$ so that: 
% \begin{equation}
% \label{eq:problem}
% \hat a =\underset{a}{\text{argmax}}\, log\, p(a\, |\, e)
% \end{equation}
% Here $log\, p(a\, |\, e)$ is estimated by the model using Equation~\ref{eq:decoding}. We define $a = a_1,...,a_m$  as an assembly code token sequence with length $|m|$. We define $e = e_1,...,e_n$ as a natural language token sequence with length $|n|$.

% \subsection{Seq2Seq Model}
% \label{subsection:model}

%In this subsection, we describe the neural sequence-to-sequence (Seq2Seq) model used for our task. As mentioned in~\ref{section:problem}, Seq2Seq learning maximizes the likelihood (or potentially other evaluation metrics \cite{shen2016minimum}) of the target sequence (assembly code tokens) given an input source sequence (English intent tokens).

%Encoder-Decoder architectures using RNNs and applied to solve Seq2Seq tasks were first proposed by \cite{cho2014learning} and \cite{sutskever2014sequence}. In practice, gated RNNs such as LSTMs \cite{hochreiter1997long} tend to perform better over vanilla RNNs \cite{gu2016incorporating}.

%With that in mind, 
%We employ an LSTM-based recurrent network encoder-decoder architecture in a \emph{seq2seq} model. 
% Similar to \cite{bahdanau2014neural} encoder-decoder architecture with attention, we use a bi-directional LSTM as the encoder to transform an embedded intent sequence $E = |e_1,...,e_{T_S}|$ into a vector $c$ of hidden states with equal length. We implement this architecture with Bahdanau-style attention \cite{bahdanau2014neural} using {\fontfamily{qcr}\selectfont xnmt} \cite{neubig2018xnmt}. We use an Adam optimizer \cite{kingma2014adam} with $\beta_1=0.9$ and $\beta_2=0.999$. The learning rate $\alpha$ is optimized and it will be described in \S~\ref{subsection:hyperparams}. The last step is inference. During inference, the \textbf{\textit{Auto Regressive Inference}} component uses beam search with a beam size of $5$. The train/dev/test split is train (N = 1,940), dev (N = 243), and test (N = 242) using an $80/10/10$ ratio.
 %This vector is known as context vector or the thought vector. 

% Each hidden state $h_t$ corresponds to
% an embedded token $e_t$ Each hidden state is computed by concatenating the hidden states of the forward and backward orders as follows:
% \begin{equation}
% \label{eq:encoding}
% \begin{matrix}
% \textbf{h}_t = [f(e_t,\textbf{h}_{t-1}) ; f(e_t,\textbf{h}_{t+1})] ;  \\ \\
% \textbf{c} = \phi(\{\textbf{h}_1, ..., \textbf{h}_{T_S}\}) 
% \end{matrix}
% \end{equation}
% where $\{h_t\}$ are hidden LSTM states, $f$ is a standard LSTM update function, and $\phi$ summarizes the hidden states. The decoder LSTM generates the target token $a$ using the conditional probability defined in Eq.~\ref{eq:decoding}.

% which takes in the context vector $c$ and generates target token $a$ at time $t$ using the following conditional probability:

% \begin{equation}
% \label{eq:decoding}
% \begin{matrix}
% \textbf{s}_t = f(a_{t-1},\textbf{s}_{t-1}, \textbf{c}) \\ \\
% \: \: \: \: \: \:  p(a_t|a_{<t},E) = g( a_{t-1},\textbf{s}_t,\textbf{c}))
% \end{matrix}
% \end{equation}
% where $s_t$ is the decoder LSTM state at time $t$, $a_t$ is the predicted assembly token at $t$ using function $g$.  $a_{<t}$ denotes previous predicted tokens $\{a_1,...,a_{t-1}\}$.\\

%Next, we describe the attention mechanism used. 

% We use the Bahdanau-style attention mechanism described in \cite{bahdanau2014neural}. %, in which it considers a dynamic context $\textbf{c}_t$ in the decoding process.  This attender attends to the entire input space (i.e. soft attention) by representing $\textbf{c}_t$ as the weighted sum of the source hidden states as follows: 
%\begin{equation}
% \label{eq:attention}
% \begin{matrix}
% \mathbf{c}_t = \sum_{i=1}^{{T_S}} \alpha_{t,i}\: \textbf{h}_i \\ \\
% %\alpha_{t,i} = \frac{\exp(score(\textbf{s}_{t-1}, \textbf{h}_i))}{\sum_{i'=1}^n \exp(score(\textbf{s}_{t-1}, \textbf{h}_{i'}))}
% \alpha_{t,i} = softmax(score(\textbf{s}_{t-1},\textbf{h}_i)) \\ \\
% score(\textbf{s}_{t},\textbf{h}_i) = v_{z}^{\top} tanh(\textbf{W}_z[\textbf{s}_t; \textbf{h}_i])
% \end{matrix}
% \end{equation}
%where $\alpha_{t,i}$ represents how well a target token $a_t$ and source token $e_i$ align, $T_S$ represents the last hidden state in $c$,  $s_t$ is the decoder LSTM state at time $t$, and lastly, $v_z$ and $W_z$ are weight matrices to be learned by the alignment model. The score $\alpha_{t,i}$  is parametrized  by a feed-forward multi-layer perceptron neural network. %Since the encoder uses a bi-directional LSTM each hidden state $\textbf{h}_i$ is aware of the context on both ends.  
% The last step is inference. During inference, the \textbf{\textit{Auto Regressive Inference}} component uses beam search with a beam size of $5$. %to approximate the best $\hat{a}$ from Eq.~\ref{eq:problem}.


% With that in mind, we employ a recurrent neural network (RNN) architecture \cite{luong2015effective} as the decoder.
% In this work, we use the neural machine translation architecture proposed by \cite{bahdanau2014neural}, and briefly summarized in the following Figure~\ref{fig:arch}. 
% %\footnote{We underline that our approach is not specific to any architecture.}. 

% The encoder is a bidirectional neural network with gated recurrent units \cite{cho2014learning} that reads an input sequence and calculates a forward sequence of hidden states, and a backward sequence. The forward sequence and the backward sequence are concatenated to obtain the annotation vector $h_j$. The decoder is a recurrent neural network that predicts a target sequence.

% The weight of each annotation $h_j$ is computed through an alignment model $\alpha_{ij}$, which models the probability that $y_i$ is aligned to $x_j$. The alignment model is a single layer feed-forward neural network that is learned jointly with the rest of the network through back-propagation. 




%  Section 4




% Programming + NLP Table

% \begin{table*}[h!]
% % \footnotesize
% \fontsize{9}{11}\selectfont
% \renewcommand{\arraystretch}{0.8}
% % \centering
% % \begin{tabular}{>{\centering\arraybackslash}m{3.7cm}|>{\centering\arraybackslash}m{3.7cm}|>{\centering\arraybackslash}m{3.7cm}}
% \begin{tabular}{p{5cm} p{9cm} b{1.5cm}}
% % \begin{tabular}{llc}
% \toprule
% \multicolumn{1}{l}{\textbf{NLP Application}}  & \multicolumn{1}{l}{\textbf{Description}}   & \multicolumn{1}{c}{ \begin{tabular}[r]{@{}r@{}}\textbf{References}  \end{tabular}  }   \\ \toprule 

% Program Synthesis   & \begin{tabular}[c]{@{}l@{}}The task of synthesizing complete or partial programs \\ given a specification, often structured input. \end{tabular} &  \\ \hline

% Program Analysis  & \begin{tabular}[c]{@{}l@{}} Focuses on extracting semantic properties\\ from programs. \end{tabular} &  \begin{tabular}[c]{@{}l@{}}   \end{tabular} \\ \hline

% Program Repair  &   \begin{tabular}[c]{@{}l@{}} Focuses on building models to repair codebases\\ given a compiler error message and a corresponding codebase. \end{tabular} &    \begin{tabular}[c]{@{}l@{}} \cite{Yasunaga20DrRepair}   \end{tabular} \\ \hline

% Clone Detection$^*$ &   \begin{tabular}[c]{@{}l@{}} Focuses on measuring the semantic similarity between \\ two  codes. There are variations of this task binary \\classification and retrieving code of semantic equivalence. \end{tabular} & \begin{tabular}[c]{@{}l@{}}   \end{tabular} \\ \hline


% Defect Detection$^*$ &   \begin{tabular}[c]{@{}l@{}}Focuses on detecting insecure code that can be exploited \\ in attacks such as DoS. The task is a binary classification \\ problem. \end{tabular} &    \begin{tabular}[c]{@{}l@{}}\cite{zhou2019devign}  \end{tabular} \\ \hline

% Cloze Test$^*$  &   \begin{tabular}[c]{@{}l@{}}Focuses on predicting the correct token in a code function \\ given a natural language description and a code function \\ with a masked token. \end{tabular} &    \begin{tabular}[c]{@{}l@{}}~\cite{husain_codesearchnet_2019,CodeXGLUE,feng_codebert_2020}   \end{tabular} \\ \hline

% Code Translation$^*$  &   \begin{tabular}[c]{@{}l@{}} Focuses on using machine learning to translate \\ source code  from a particular language (e.g. Python) \\ to another language (e.g. JavaScript). \\ Also known as Code Transpiling. \end{tabular} &    \begin{tabular}[c]{@{}l@{}} \cite{lachaux2020unsupervised}   \end{tabular} \\ \hline

% Code Refinement$^*$  &   \begin{tabular}[c]{@{}l@{}}Focuses on automatically fixing bugs in a given codebase. \end{tabular} &    \begin{tabular}[c]{@{}l@{}}\cite{tufano2019empirical}  \end{tabular} \\ \hline

% Code Completion$^*$  &   \begin{tabular}[c]{@{}l@{}} Focuses on generating a code snippet \\ that best completes a given program. \end{tabular} &    \begin{tabular}[c]{@{}l@{}}   \end{tabular} \\ \hline

% Code Search and Retrieval$^*$  &   \begin{tabular}[c]{@{}l@{}} Retrieve a code snippet given a natural language query. \end{tabular} &   \begin{tabular}[c]{@{}l@{}}   \end{tabular} \\ \hline

% Code Documentation Generation$^*$  &   \begin{tabular}[c]{@{}l@{}} Generating natural language descriptions \\ for code snippets. \end{tabular} &    \begin{tabular}[c]{@{}l@{}}   \end{tabular} \\ \hline

% Documentation Translation$^*$  &   \begin{tabular}[c]{@{}l@{}}Focuses on translating online code doc pages \\ from one human language to another. \end{tabular} &    \begin{tabular}[c]{@{}l@{}} \cite{CodeXGLUE}  \end{tabular} \\ \hline

%  \begin{tabular}[c]{@{}l@{}} Code Generation from \\ Natural Language$^*$ \end{tabular}  &   \begin{tabular}[c]{@{}l@{}} Generating code snippets given \\  natural language intents. \end{tabular} &    \begin{tabular}[r]{@{}r@{}} \cite{yin_tranx_2018} \end{tabular} \\ \hline

% Semantic Parsing  &   \begin{tabular}[c]{@{}l@{}} Converting natural language to \\ unambiguous executable logical forms.\end{tabular} &     \begin{tabular}[c]{@{}l@{}}   \end{tabular} \\ 

% \bottomrule
% \footnotesize{$^*$ Included in CodeXGLUE}.
% \end{tabular}
% \caption{Overview of application areas of Natural Language Processing on source code.}
% \label{nlp_code}
% \end{table*}


%  Summary of big code

% \ea{TODO: Cite References}
% The logio-deductive approach proves facts and properties of a program by conceiving software tools in formal terms. The availability of “big-code” facilitated the usage of statistical and deep learning data-driven models as approaches to developing software tools. The naturalness hypothesis holds that coding is an act of communication thus it is exploitable using probabilistic ML methods. The naturalness hypothesis drives the research area to exploit the statistics of code by creating probabilistic source code models that learn how coders write and use code. These methods also enable learning correspondences between code and requirements, blog posts, and comments etc. Code predictability denotes that source code contain useful predictable patterns. Uncertainty in code is not common because code is unambiguous however, natural text components, such as comments are ambiguous. Hence it is necessary to deal with uncertainty in the domain due to the correspondence between unambiguous code and ambiguous text. Source code is bimodal and is less ‘surprising’ and more predictable than text. All code have the following properties: Executability, Formality, and Cross-Channel Interaction. Codes have two units, algorithmic units consisting of loops operations etc, and semantic units such as identifiers, statements and blocks. Probabilistic machine learning models make simplifying assumptions to make the models tractable to learn and use, however they become erroneous. There are three different types of probabilistic models in the related works: Code-Generating models, Representational Models of Code, and Pattern Mining Models. Code-generating models define a probability distribution over code by modeling the generation of smaller parts of code such as Abstract Syntax Tree Nodes. These models rely on Naive Bayes and consist of n-gram models mainly and use the probability of each possible snippet as a scoring function with smoothing (no zero probabilities). These models do not generate syntactically correct code or code that always compiles and does not take into account the context strongly such as scope. RNNs outperform n-gram language models. They loosen the fixed context-size assumption. RNNs perform better due to their hidden state, it can encode longer-range dependencies of contexts and they can learn similarities across contexts. Syntactic models, which is what we use in EnPy, generate code at the level of Abstract Syntax Trees. The strength of these models lie in their ability to generate syntactically correct code (it does not mean that it compiles though). Also graphs were used to represent code semantics however, generating complex graphs is still hard because they do not have a natural starting point. Code Transducer models translate code from one format into another. It’s been generally applied in code migration, pseudocode generation, and code fixing. There are also multi modal models that correlate code with one or more non-code modalities. Reference 23,51, and 55 designed a model that accepts visual input and generates a code in DSL describing how the input was constructed. Applications of Big Code in recommender systems  include making snippet recommendations to assist in software engineering tasks such as auto-completion, recommending code reviewers for a code change, and suggesting names for variables, methods, and classes by using relevant code tokens as the context (References 5,6,10). Other applications include inferring the emergent coding conventions from an inputted source code, finding code defects, and code translation where codes are translated from one language (Java for example) to another (C\#).  Code to Text and Text to Code includes linking natural language text to source code. It has many useful applications such as program synthesis, trace-ability, search and documentation. This problem is difficult due to the compositional nature of the code and the ambiguity of the corresponding natural language. Text to code aims to help people and developers write programs more easily.





% \begin{figure*}[t!]
%   \includegraphics[width=\linewidth]{figures/fig1.jpg}
%   \caption{Dialogue manager control flow from Serban et al.~\citeyearpar{serban_deep_2017}.}
%   \
%   \label{fig:flow}
% \end{figure*}


% MILABOT is a participating chatbot bot in the 2017 iteration of the Amazon Socialbot Grand Challenge, that converses through Amazon’s Echo device by generating "a candid set of dialogue responses" as the \textbf{output} given a human dialogue \textbf{input} in both speech and text \cite{serban2017deep}. MILA participates in the Alexa Socialbot challenge and scores 3.15 in user ratings \cite{serban2017deep}. MILABOT is comprised of 22 different response systems, with each system generating a response given human dialogue input. MILABOT applies a reinforcement learning mechanism to select the most appropriate response. In this report, I discuss the MILABOT system overall along with its model selection policy and analyze the response systems \textit{AliceBot}, \textit{InitiatorBot}, and \textit{Evibot} within MILABOT further in depth. 


% \subsection{Pseudocode}
% In this section, I explain how MILABOT chooses an appropriate response, further discuss the psuedocodes of two specific template-based models  \textit{AliceBot} and \textit{InitiatorBot},  briefly describe \textit{StoryBot}, and discuss the pseudocode of \textit{EviBot} a knowledge base-based question answering model. Human language is complex, to where it nearly impossible to encode rules for carrying out human conversations. MILABOT uses an ensemble of 22 response models including, generation-based neural networks, retrieval-based neural networks, knowledge base question answering systems and template-based systems \cite{serban2017deep}. Each of these response models take in human dialogue input and generate a response in text. MILABOT uses a reinforcement learning mechanism to select an appropriate response from the array of response models it has.

% \subsection{\label{sec:conv_approaches}Conversational AI Approaches}
% In this section, I explain the \textit{dialogue manager} component which is a crucial component in MILABOT's response generation and selection mechanism. The \textit{dialogue manager} combines all of the 22 response models together mentioned earlier. It uses all the utterances recorded in the dialogue throughout the conversation, including the current utterance, and the confidence values of text transcriptions from the automatic speech recognition system (ASR) as \textbf{input}. The \textit{dialogue manager} follows a three-step procedure, first it generates a set of candidate responses using all 22 response models in its ensemble. The \textit{dialogue manager} then checks to see if there is a generated response flagged as a \textit{priority response}, which is a response flagged by the response models themselves under certain encoded circumstances, the \textit{dialogue manager} returns the priority response automatically. If there are no priority responses, the dialogue manager selects the appropriate response using the \textit{model selection policy} which will be discussed later. The processes of the dialogue manager are illustrated in Figure~\ref{fig:flow}.

% \begin{figure*}[t!]
%   \includegraphics[width=\linewidth]{figures/fig1.jpg}
%   \caption{Dialogue manager control flow from Serban et al \cite{serban_deep_2017}.}
%   \
%   \label{fig:flow}
% \end{figure*}

% \subsection{Model Selection Policy}
% This section describes the model selection policy which is used by the dialogue manager mentioned in section~\ref{sec:dm} to select an appropriate response. An appropriate response is defined as "a response which increases the  satisfaction of the user for the entire dialogue" \cite{serban_deep_2017}. The \textit{model selection policy} uses the reinforcement learning framework, in which an agent takes actions in an environment in order to maximize rewards \cite{sutton_reinforcement_1998}.  In this case, the dialogue manager is the agent, $t$ is a time step from $t = 1,...,T$. The set of actions $K$, is the set of candidate responses from the response models, and the reward, $r_t$ is the predicted user satisfaction score at time step $t$, based on the dialogue history $h_t$. The agent receives a reward $r_t$, after taking an action (choosing a particular response) from the set of possible actions $K$: $a^1_t,...,a^{22}_t$, where 22 denotes the number of response models in MILABOT. The dialogue manager's goal is to maximize the discounted sum of rewards (also known as \textit{expected cumulative return}) as denoted by the formula below:

% \begin{equation}
% 		R =  \sum_{t=1}^{T}\gamma^tr_t
% \end{equation}
% $\gamma \in {(0,1]}$ denotes the discount factor.

% \subsection{Conversational Models}
% \subsubsection{Template-Based Models}
% This section discusses the following template-based models in MILABOT: \textit{Alicebot}, \textit{Initiatorbot}, and \textit{Storybot}. \textit{Alicebot}\footnote{\url{https://www.chatbots.org/chatbot/a.l.i.c.e/}} uses a set of templates written in AIML (artificial intelligence markup language) to produce textual responses given a dialogue history and user utterance \cite{wallace_anatomy_2009,shawar_chatbots_2007}.  Alicebot generates non-priority responses, except templates related to MILABOT's name, age, and location. Basically, \textit{Alicebot} takes in input and goes through the templates in AIML and generates a template response. All responses are non-priority except responses related to age, name, and location. \textit{Alicebot} also computes a confidence score for each of its responses through string-based rules to determine if the the response composes a "correct sentence". The paper doesn't describe how a sentence is determined to be "correct". High confidence of 1.0 is given when a sentence is correct and the response is given a priority. A confidence of 0.5 is given when the sentence is correct but the response is not flagged as a priority. A confidence of 0 is given if the sentence is not correct. The full process is illustrated in Algorithm~\ref{alg:alice}.\vspace{0.5cm}

% \begin{algorithm}[h!]
% \SetAlgoLined
%     \textbf{input: } dialogue history
%     \BlankLine
%     response $\leftarrow$ apply AIML templates to dialogue history
%     \BlankLine
%  \eIf{\textit{response is correct sentence}}{
%   \eIf{\textit{response is given priority}}{
%   confidence $\leftarrow$ 1.0
%   }{
%     confidence $\leftarrow$ 0.5
%   }
%   }
%   {
%   confidence $\leftarrow$ 0.0
   
%   }
%   \textbf{output: } response, priority, confidence
%  \caption{\label{alg:alice}Alicebot from Serban et al \cite{serban_deep_2017}}
% \end{algorithm}

% \vspace{0.3cm}
% \begin{algorithm}[h!]
% \SetAlgoLined
%     \textbf{input:} dialogue history
%     \BlankLine
    
%      \uIf{Initiatorbot was triggered in one of last two turns}{
%         return ""
   
%   }
    
%     \uElseIf{user did not give a greeting}
%         {
%             return a non-priority response with a random initiator phrase
%         }
   
%   \Else{
%   return a priority response with a random initiator phrase
   
%   }
%   \textbf{output: } response, priority, confidence
%  \caption{\label{alg:ini}Initiatorbot from Serban et al \cite{serban_deep_2017}}
% \end{algorithm}
% \vspace{0.3cm}





% %\ref{alg:ini}
% %\ref{alg:alice}
% % Talk about pseudocodes a little bit
% \vspace{0.3cm}
% \textit{Initiatorbot} model is a conversation starter. It intends to engage the user with open-ended questions to get the conversation started. \textit{Initiatorbot} pulls from a bank of 40 written questions such as "\textit{What did you do today?"} Occasionally, the model can also initiate the conversation by mentioning an interesting fact from a database of interesting facts. This response model is triggered when the user mentions a greeting. When the user greets MILABOT, \textit{Initiatorbot} gets priority and responds with a question, enabling MILABOT to take control (initiative) of the conversation or dialogue. The paper does not report  how many greetings they have in their list of greetings. The initiation phrases and questions are picked randomly from all possible initiation phrases. The process is further illustrated in Algorithm~\ref{alg:ini}.
% % Talk about storybot
% \textit{Storybot}, is a response model in MILABOT that tells a short fiction story, when the user requests it. This response model s given priority only when the user's utterance includes a request word, (e.g. \textit{say, tell, share}) and a word related to stories (e.g. \textit{story, tale, narrative}. The paper does not mention how many request keywords nor how many story-type words they use for trigger purposes hence, $n$ is missing for both. \textit{Storybot}, responds with a story's title, author, and then story body. The stories were compiled from: \url{www.english-for-students.com}. If the response is not a priority from \textit{Storybot}, MILABOT doesn't use it.


% \subsubsection{Knowledge Base-based Question Answering}
% \begin{algorithm}[h!]
% \SetAlgoLined
%     \textbf{input:} dialogue history
%     \BlankLine
%      query $\leftarrow$ last utterance
%      \BlankLine
%      has-wh-words $\leftarrow$ true if utterance contains a wh-word, otherwise false
%     \BlankLine
%      has-only-stop-words $\leftarrow$ true if utterance has only stop words, otherwise false
%     \BlankLine
%      \uIf{has-only-stop-words and not has-wh-words}{
%         return ""
   
%   }
%     \BlankLine
%     evi-response $\leftarrow$ send query to \url{www.evi.com}
%     \BlankLine
%     priority $\leftarrow$ true if has-wh-words and evi-response is valid otherwise false 
%       \BlankLine
%     \uIf{evi-response is valid}
%         {
%             return evi-response, priority
%         }
        
%          \uElseIf{has-wh-words}
%         {
%               priority $\leftarrow$ has-wh-words
%               subentities $\leftarrow$ entities extracted from query using NLTK's named entity processor
%               subphrases $\leftarrow$ list of subphrases with entities
%               \BlankLine
%               \For{subphrase in subphrases}
%               {
%               		evi-response $\leftarrow$ send subphrase to \url{www.evi.com}
%                     \uIf{evi-response is valid}
%                     {
%                     	return evi-response, priority
%                     }
%               }
%               \BlankLine
%                  subphrases $\leftarrow$ list of subphrases
%                   \BlankLine
%                   \For{subphrase in subphrases}
%               {
%               		evi-response $\leftarrow$ send subphrase to \url{www.evi.com}
%                     \uIf{evi-response is valid}
%                     {
%                     	return evi-response, priority
%                     }
%               }
               
%         }
        
   
%   \Else{
%   return ""
%   }
%  \caption{\label{alg:evi}Evibot from Serban et al \cite{serban_deep_2017}}
% \end{algorithm}
% \vspace{0.3cm}

% \textit{Evibot} is a MILABOT response model, that answers questions using an Amazon question-answering web-service \textit{Evi}: \url{www.evi.com}. \textit{Evibot}'s responses are flagged as priority when the user's utterance contains a wh-word (e.g. \textit{what},\textit{who},\textit{where}). \textit{Evibot} returns an answer to the user's question. To generate the response \textit{Evibot} follows a three-step procedure. The response model first sends the user utterance holistically to the web-service and returns the results answer if it is "valid" (valid is not defined in the referenced paper). If the query to the web-service fails, the answer is empty, or the answer is invalid, \textit{Evibot} uses NLTK's named entity module \cite{bird_natural_2009} to find the named entities in the user utterance.  Then it it creates a sub-query for each named entity in the user utterance and sends it to the web-service and then returns the result if the response is valid. If both steps above fail, \textit{Evibot}, sends the  queries to the web-service containing all sub-queries without named entities and either returns a valid response or an empty response. The full process is illustrated in Algorithm~\ref{alg:evi}.

% \subsubsection{Alexa Socialbot Challenge}
% This section, discusses competing algorithms in template-based bots and then discuss other Alexa socialbots, comparing the similarities and discussing the novelties and differences of each along the way. \textit{Alicebot} and \textit{Initiatorbot}  are amongst many different template-based text generators that interact with users. All template-based bots are similar to Elizabot, a bot that performs string-matching to select an answer from a set of templates \cite{weizenbaum1966eliza}. Elizabot specifically mimics a psychotherapist and attempts to engage the user in a conversation about themselves. \textit{Initiatorbot} is specifically designed to initiate conversations only by asking open-ended questions, it has a specific role in a conversation and cannot stand alone by itself. On the other hand, \textit{Alicebot} also performs string matching however, it's build using AIML and has more templates than Elizabot. It also computes a confidence score for it's responses based on whether the sentence is correct or not.
% % Talk about novelty of MILABOT
% The novelty of MILBOT as a system, is in its large-scale usage of ensemble machine learning and deep learning models with a reinforcement learning selection mechanism. The model scores 3.15 out of 5 in user satisfaction which above the average of 2.92 \cite{serban2017deep}. The model is also very likely to improve given more interactions due to its reinforcement learning architecture. Slugbot, an Alexa socialbot competitor, is composed of a modular system using the human mind as a model for data management \cite{bowden2018slugbot}. Slugbot also attempts to generate its own opinions, however, the methods employed in Slugbot for curating opinions is reported to be extremely inefficient \cite{bowden2018slugbot}. Alquist 2.0, is another participating Alexa socialbot in 2018. It's novelty lies in its leveraging ontology-based topic structures and the way the conversation is modeled into sub-dialogues enhancing the uniqueness of each session \cite{pichi2018alquist}. Lastly, Emersonbot is another competing socialbot in 2017. It's novelty lies in its federated multi-source information retrieval system that is context-aware whilst conversing; a machine-learning based dialogue management system, complemented with rule-based conversational logic components \cite{wang2017emersonbot}. Each of these social bots is a unique system with its own pros and cons that provides a unique experience to its conversing users.



% Talk about other related works (Other Alexa competitors?) Would need citations

% % Look at citations of AliceBot and talk about bank of america erica and customer service bots etc
% Conversational Artificial Intelligence is is an on-going problem and an active area of research where machines are enabled to have free-form conversations in a wide array of domains and topics \cite{ram2018conversational}. Applications of such socialbots include autonomous operations on social media networks, influencing and transforming relationships among people and organizations on those sites \cite{hwang2012socialbots}. A double-edged sword, a lone socialbot, could significantly change in a behavior of an entire social group, furthermore, a larger group of bots, can reshape entire communities at a larger scale in what experts call "social architecting" \cite{hwang2012socialbots}. Such influence, could facilitate increasing friendship rates through introducing users to each other \cite{hwang2012socialbots}, large scale manipulation of online information, opinion distortion, and data theft from institutions \cite{bakardjieva2015rationalizing}. Conversational bots are also used as search interfaces offering an alternative search modality \cite{d2017artificial} such as \textit{Erica} in the Bank of America mobile app. Research findings suggest that users are more likely to share personal information while interacting with a machine interface \cite{tantam2006machine}. Hence, conversational socialbots could be used to "guide a user in terms of disclosing emotions, therapy preferences and needs" \cite{d2017artificial}.  Socialbots are a double-edged sword with various applications. They spark a worldwide ethical debate as the field of Conversational Artificial Intelligence advances.

% \subsubsection{Applications in Software Engineering}
% Talk about applications and corresponding evaluation methods.

% \subsubsection{Applications in Education}
% Talk about applications and corresponding evaluation methods.
